Know Your Limits: A Survey of Abstention in Large Language Models

Abstention, the refusal of large language models (LLMs) to provide an answer, is increasingly recognized for its potential to mitigate hallucinations and enhance safety in LLM systems. In this survey, we introduce a framework to examine abstention from three perspectives: the query, the model, and human values. We organize the literature on abstention methods, benchmarks, and evaluation metrics using this framework, and discuss merits and limitations of prior work. We further identify and motivate areas for future research, such as whether abstention can be achieved as a meta-capability that transcends specific tasks or domains, and opportunities to optimize abstention abilities in specific contexts. In doing so, we aim to broaden the scope and impact of abstention methodologies in AI systems.

==> tables/method.tex <==
\begin{figure*}[h!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            [
               Abstention methods in LLMs, ver, 
               color=black!100, fill=black!15,
                text=black
                [
                    Pretraining, color=yellow!100, fill=yellow!100, text width=4.0em, text=black
                    [
                        Data augmentation, color=yellow!100, fill=yellow!60,  text width=7.0em, text=black
                        [
                            \citet{neeman2022disentqa}, cause_leaf, text width=27.5em
                        ]
                    ]
                       
                ]
                [
                    Alignment, color=cyan!100, fill=cyan!100, text width=4.0em, text=black
                    [
                        Instruction tuning, color=cyan!100, fill=cyan!60,  text width=7.0em, text=black
                        [
                            \citet{zhang2023r, yang2023alignment, chen2023adaptation, feng2024don} \\ \citet{bianchi2023safety,varshney2023art, wallace2024instruction} \\
                            \citet{zhang2023defending, lyu2024keeping, wang2023self}
, cause_leaf, text width=27.5em
                        ]                        
                    ]

                    [
                        Learning from \\ preferences, color=cyan!100, fill=cyan!60,  text width=7.0em, text=black
                        [
                            \citet{cheng2024ai, liang2024learning, lin2024flame, guo2024controllable} \\
\citet{zhang2024selfalignment, dai2023safe, touvron2023llama} \\
\citet{bai2022training, shi2024saferinstruct, kim2024break, sun2024salmon}, cause_leaf, text width=27.5em
                        ]
                    ]
                    
                       
                ]
                

                
                
                [
                    Inference, color=lightgreen!200, fill=lightgreen!200, text width=4.0em, text=black
                    [
                            Input-processing, color=lightgreen!150, fill=lightgreen!150, text width=7em, text=black  [
                                % Malicious Query \\ Detraction, 
                                Query processing,
                                color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{qi2020onion, hu2024tokenlevel, sun2023defending, dinan2019build} \\
\citet{jain2023baseline, shao2021bddr, kumar2024certifying, xi2024defending}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            
                    ]
                       [
                            In-processing , color=lightgreen!150, fill=lightgreen!150, text width=7em, text=black
                            [
                                Probing LLM’s \\ inner state, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{kamath2020selective, azaria2023internal, slobodkin-etal-2023-curious} \\
\citet{kadavath2022language, liu2020simple, chen2024inside} \\
\citet{wang2024inferaligner, bhardwaj2024language}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            [
                                Uncertainty \\ estimation, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{lin2022teaching, tian2023just, tomani2024uncertainty} \\
\citet{kadavath2022language, kuhn2023semantic, xiong2023can} \\
\citet{cole2023selectively, achiam2023gpt, ren2023self} \\
\citet{duan2023shifting, shrivastava2023llamas}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            [
                                Calibration-based, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{zhao2022calibrating,xiao2022uncertainty,jiang2021can}, \\
\citet{varshney2022investigating,mielke2022reducing,lu2022learning}, \\
\citet{clark2020electra,wen2020batchensemble,desai2020calibration}, \\
\citet{zablotskaia2023uncertainty,hou2023decomposing}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            [
                                Consistency-based, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{slobodkin-etal-2023-curious,xiong2023can,kadavath2022language}, \\
\citet{lin2024generating,cole2023selectively,robey2023smoothllm}, \\
\citet{cao2023defending,ji2024defending,yuan2024rigorllm}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            [
                                In-context learning, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{slobodkin-etal-2023-curious, wen2024characterizing, yang2023alignment} \\
\citet{cheng2024ai, kadavath2022language, ren2023self} \\
\citet{lin2024generating, varshney2023art, wei2024jailbreak} \\
\citet{mo2024studious, zhou2024robust, pisano2023bergeron} \\
\citet{zhang2023defending, zhang2024intention, xie2023defending, zhou2024defending}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                       ]
                       [
                            Output-processing, color=lightgreen!150, fill=lightgreen!150, text width=7em, text=black
                            [
                                Self evaluation, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{helbling2023llm, kadavath2022language, varshney2023art} \\
\citet{ren2023self, wang2024selfguard}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                            [
                                LLM collaboration, color=lightgreen!100, fill=lightgreen!60,  text width=7.0em, text=black
                                [
                                    {\citet{mielke2022reducing, wang2024selfguard, pisano2023bergeron} \\
                                     \citet{feng2024don, zeng2024autodefense,chen2023jailbreaker}
}, cause_leaf, text width=25.5em
                                ]
                                
                            ]
                        ]
                ]
            ]   
            
        \end{forest}
        }
\caption{Methods to improve LLM abstention ability categorized by pretraining, alignment, and inference stages.}
\label{fig:categorization_of_survey}
\end{figure*}
